TIES: Temporal Interaction Embeddings For Enhancing Social Media Integrity At Facebook

Since its inception, Facebook has become an integral part of the online social community. People rely on Facebook to make connections with others and build communities. As a result, it is paramount to protect the integrity of such a rapidly growing network in a fast and scalable manner. In this paper, we present our efforts to protect various social media entities at Facebook from people who try to abuse our platform. We present a novel Temporal Interaction EmbeddingS (TIES) model that is designed to capture rogue social interactions and flag them for further suitable actions. TIES is a supervised, deep learning, production ready model at Facebook-scale networks. Prior works on integrity problems are mostly focused on capturing either only static or certain dynamic features of social entities. In contrast, TIES can capture both these variant behaviors in a unified model owing to the recent strides made in the domains of graph embedding and deep sequential pattern learning. To show the real-world impact of TIES, we present a few applications especially for preventing spread of misinformation, fake account detection, and reducing ads payment risks in order to enhance the platform's integrity.

==> sections/related_work.tex <==
\section{Related Work}~\label{sec:related_work}



\begin{figure*}[t]
	\centering
	\includegraphics[width=0.95\linewidth]{figs/ties-model1}
	\caption{TIES Model Architecture}
	\label{fig:ties-model1}
\end{figure*} 

There is a large literature on fake account detection in online social networks.  Previous work in the area of fake account detection has focused on utilizing graph and neighbor based features in graph propagation style algorithms.  ~\cite{yang2012analyzing} use graph propagation to detect spammers on Twitter over a user following graph.  Integro~\cite{boshmaf2015integro} focuses on predicting “victims” using user-level features and performs a random walk style algorithm on a modified graph.  There have been other works that focus on utilizing the graph structure, by identifying cohorts of malicious actors that share common IP addresses and other common networking properties~\cite{stringhini2015evilcohort} or by creating an activity graph and identifying tightly connected components to detect malicious actors (Zhao et al.~).  An alternate route to create graph is based on user activity and have been exploited to detect fake engagments~\cite{li2016world}. Similarly features engineered by hand based on activity has been in~\cite{chen2018fakebuster} for the same purpose.   Still other works examined propagation patterns of spam~\cite{nilizadeh2017poised}.   Several clustering techniques based approach have also been proposed to detect fake accounts such as in~\cite{xiao2015detecting}.

Still other methodologies in fake account detection incorporate a number of graph and behavioral features in a multi-stage multi-task learning framework (DEC paper).  

Our work differs from these previous works in that we use an embedding based methodology over the sequence of interactions between a source user and any number of target users.  There has been previous work in the field of temporal interaction networks and embeddings.~\cite{kumar2019predicting} present JODIE, a novel embedding technique to earn joint user and item embeddings from sequential data.  While these authors apply their algorithm to the problem of detecting bans from Wikipedia and Reddit, which is similar to the problem of fake account detection, their work is different from ours in a number of ways.  Namely, they are applying two RNNs to learn joint user-item embeddings based on temporal interaction sequences, while we just want to learn the embedding for the source account in the interaction based on the temporal sequence.  In order to leverage the target accounts’ current state, we use pre-existing embeddings that are trained on interaction data, but not necessarily in a temporal way.  Another difference between JODIE and our work introduces a projection operator that learns to estimate the embedding of the user at any time in the future in order to predict future user-item interactions.  Despite the differences between our paper and JODIE, we provide an analysis of the performance of both algorithms in the experimental section of this paper. 



==> sections/results.tex <==
\section{Results}~\label{sec:results}
...
